Study of the Dalitz decay $J/\psi \to e^+e^- \eta$

We report corrected results on a study of the electromagnetic Dalitz decay $J/\psi \to e^+e^- \eta$ and search for di-electron decays of a light dark gauge boson ($\gamma'$) in $J/\psi \to \gamma' \eta$ with the two $\eta$ decay modes $\eta \rightarrow \gamma \gamma$ and $\eta \rightarrow \pi^+\pi^-\pi^0$, using $(1310.6\pm 7.0)\times10^6$ $J/\psi$ events collected with the BESIII detector. In particular we update the measurement of the pole mass of the transition form factor (TFF) of $J/\psi \to e^+e^- \eta$ to be $\Lambda = 2.56 \pm 0.04({\rm stat}) \pm 0.03({\rm syst})$ GeV/$c^2$. The branching fraction of $J/\psi \to e^+e^-\eta$ and the kinetic-mixing strength between the Standard Model photon and $\gamma'$ are also updated after taking the corrected $\Lambda$ value into account. The measured branching fraction of $J/\psi \to e^+e^- \eta$ is updated to be $(1.42 \pm 0.04({\rm stat}) \pm 0.07 ({\rm syst}))\times 10^{-5}$, where the first and second uncertainties are statistical and systematic, respectively.

==> author.tex <==
\author{\small
M.~Ablikim$^{1}$, M.~N.~Achasov$^{10,b}$, P.~Adlarson$^{68}$, S. ~Ahmed$^{14}$, M.~Albrecht$^{4}$, R.~Aliberti$^{28}$, A.~Amoroso$^{67A,67C}$, M.~R.~An$^{32}$, Q.~An$^{64,50}$, X.~H.~Bai$^{58}$, Y.~Bai$^{49}$, O.~Bakina$^{29}$, R.~Baldini Ferroli$^{23A}$, I.~Balossino$^{24A}$, Y.~Ban$^{39,h}$, K.~Begzsuren$^{26}$, N.~Berger$^{28}$, M.~Bertani$^{23A}$, D.~Bettoni$^{24A}$, F.~Bianchi$^{67A,67C}$, J.~Bloms$^{61}$, A.~Bortone$^{67A,67C}$, I.~Boyko$^{29}$, R.~A.~Briere$^{5}$, A.~Brueggemann$^{61}$, H.~Cai$^{69}$, X.~Cai$^{1,50}$, A.~Calcaterra$^{23A}$, G.~F.~Cao$^{1,55}$, N.~Cao$^{1,55}$, S.~A.~Cetin$^{54A}$, J.~F.~Chang$^{1,50}$, W.~L.~Chang$^{1,55}$, G.~Chelkov$^{29,a}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,55}$, M.~L.~Chen$^{1,50}$, S.~J.~Chen$^{35}$, X.~R.~Chen$^{25}$, Y.~B.~Chen$^{1,50}$, Z.~J.~Chen$^{20,i}$, W.~S.~Cheng$^{67C}$, G.~Cibinetto$^{24A}$, F.~Cossio$^{67C}$, J.~J.~Cui$^{42}$, X.~F.~Cui$^{36}$, H.~L.~Dai$^{1,50}$, J.~P.~Dai$^{71}$, X.~C.~Dai$^{1,55}$, A.~Dbeyssi$^{14}$, R.~ E.~de Boer$^{4}$, D.~Dedovich$^{29}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{28}$, I.~Denysenko$^{29}$, M.~Destefanis$^{67A,67C}$, F.~De~Mori$^{67A,67C}$, Y.~Ding$^{33}$, C.~Dong$^{36}$, J.~Dong$^{1,50}$, L.~Y.~Dong$^{1,55}$, M.~Y.~Dong$^{1,50,55}$, X.~Dong$^{69}$, S.~X.~Du$^{73}$, P.~Egorov$^{29,a}$, Y.~L.~Fan$^{69}$, J.~Fang$^{1,50}$, S.~S.~Fang$^{1,55}$, Y.~Fang$^{1}$, R.~Farinelli$^{24A}$, L.~Fava$^{67B,67C}$, F.~Feldbauer$^{4}$, G.~Felici$^{23A}$, C.~Q.~Feng$^{64,50}$, J.~H.~Feng$^{51}$, M.~Fritsch$^{4}$, C.~D.~Fu$^{1}$, Y.~N.~Gao$^{39,h}$, Yang~Gao$^{64,50}$, I.~Garzia$^{24A,24B}$, P.~T.~Ge$^{69}$, C.~Geng$^{51}$, E.~M.~Gersabeck$^{59}$, A~Gilman$^{62}$, K.~Goetzen$^{11}$, L.~Gong$^{33}$, W.~X.~Gong$^{1,50}$, W.~Gradl$^{28}$, M.~Greco$^{67A,67C}$, L.~M.~Gu$^{35}$, M.~H.~Gu$^{1,50}$, C.~Y~Guan$^{1,55}$, A.~Q.~Guo$^{25}$, A.~Q.~Guo$^{22}$, L.~B.~Guo$^{34}$, R.~P.~Guo$^{41}$, Y.~P.~Guo$^{9,g}$, A.~Guskov$^{29,a}$, T.~T.~Han$^{42}$, W.~Y.~Han$^{32}$, X.~Q.~Hao$^{15}$, F.~A.~Harris$^{57}$, K.~K.~He$^{47}$, K.~L.~He$^{1,55}$, F.~H.~Heinsius$^{4}$, C.~H.~Heinz$^{28}$, Y.~K.~Heng$^{1,50,55}$, C.~Herold$^{52}$, M.~Himmelreich$^{11,e}$, T.~Holtmann$^{4}$, G.~Y.~Hou$^{1,55}$, Y.~R.~Hou$^{55}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,55}$, J.~F.~Hu$^{48,j}$, T.~Hu$^{1,50,55}$, Y.~Hu$^{1}$, G.~S.~Huang$^{64,50}$, L.~Q.~Huang$^{65}$, X.~T.~Huang$^{42}$, Y.~P.~Huang$^{1}$, Z.~Huang$^{39,h}$, T.~Hussain$^{66}$, N~H\"usken$^{22,28}$, W.~Ikegami Andersson$^{68}$, W.~Imoehl$^{22}$, M.~Irshad$^{64,50}$, S.~Jaeger$^{4}$, S.~Janchiv$^{26}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{15}$, X.~B.~Ji$^{1,55}$, X.~L.~Ji$^{1,50}$, Y.~Y.~Ji$^{42}$, H.~B.~Jiang$^{42}$, X.~S.~Jiang$^{1,50,55}$, J.~B.~Jiao$^{42}$, Z.~Jiao$^{18}$, S.~Jin$^{35}$, Y.~Jin$^{58}$, M.~Q.~Jing$^{1,55}$, T.~Johansson$^{68}$, N.~Kalantar-Nayestanaki$^{56}$, X.~S.~Kang$^{33}$, R.~Kappert$^{56}$, M.~Kavatsyuk$^{56}$, B.~C.~Ke$^{73}$, I.~K.~Keshk$^{4}$, A.~Khoukaz$^{61}$, P. ~Kiese$^{28}$, R.~Kiuchi$^{1}$, R.~Kliemt$^{11}$, L.~Koch$^{30}$, O.~B.~Kolcu$^{54A}$, B.~Kopf$^{4}$, M.~Kuemmel$^{4}$, M.~Kuessner$^{4}$, A.~Kupsc$^{37,68}$, M.~ G.~Kurth$^{1,55}$, W.~K\"uhn$^{30}$, J.~J.~Lane$^{59}$, J.~S.~Lange$^{30}$, P. ~Larin$^{14}$, A.~Lavania$^{21}$, L.~Lavezzi$^{67A,67C}$, Z.~H.~Lei$^{64,50}$, H.~Leithoff$^{28}$, M.~Lellmann$^{28}$, T.~Lenz$^{28}$, C.~Li$^{40}$, C.~H.~Li$^{32}$, Cheng~Li$^{64,50}$, D.~M.~Li$^{73}$, F.~Li$^{1,50}$, G.~Li$^{1}$, H.~Li$^{44}$, H.~Li$^{64,50}$, H.~B.~Li$^{1,55}$, H.~J.~Li$^{15}$, H.~N.~Li$^{48,j}$, J.~L.~Li$^{42}$, J.~Q.~Li$^{4}$, J.~S.~Li$^{51}$, Ke~Li$^{1}$, L.~K.~Li$^{1}$, Lei~Li$^{3}$, P.~R.~Li$^{31,k,l}$, S.~Y.~Li$^{53}$, T. ~Li$^{42}$, W.~D.~Li$^{1,55}$, W.~G.~Li$^{1}$, X.~H.~Li$^{64,50}$, X.~L.~Li$^{42}$, Xiaoyu~Li$^{1,55}$, Z.~Y.~Li$^{51}$, H.~Liang$^{27}$, H.~Liang$^{1,55}$, H.~Liang$^{64,50}$, Y.~F.~Liang$^{46}$, Y.~T.~Liang$^{25}$, G.~R.~Liao$^{12}$, L.~Z.~Liao$^{1,55}$, J.~Libby$^{21}$, A. ~Limphirat$^{52}$, C.~X.~Lin$^{51}$, D.~X.~Lin$^{25}$, T.~Lin$^{1}$, B.~J.~Liu$^{1}$, C.~X.~Liu$^{1}$, D.~~Liu$^{14,64}$, F.~H.~Liu$^{45}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$, G.~M.~Liu$^{48,j}$, H.~M.~Liu$^{1,55}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{16}$, J.~B.~Liu$^{64,50}$, J.~L.~Liu$^{65}$, J.~Y.~Liu$^{1,55}$, K.~Liu$^{1}$, K.~Y.~Liu$^{33}$, Ke~Liu$^{17}$, L.~Liu$^{64,50}$, M.~H.~Liu$^{9,g}$, P.~L.~Liu$^{1}$, Q.~Liu$^{69}$, Q.~Liu$^{55}$, S.~B.~Liu$^{64,50}$, T.~Liu$^{9,g}$, T.~Liu$^{1,55}$, W.~M.~Liu$^{64,50}$, X.~Liu$^{31,k,l}$, Y.~Liu$^{31,k,l}$, Y.~B.~Liu$^{36}$, Z.~A.~Liu$^{1,50,55}$, Z.~Q.~Liu$^{42}$, X.~C.~Lou$^{1,50,55}$, F.~X.~Lu$^{51}$, H.~J.~Lu$^{18}$, J.~D.~Lu$^{1,55}$, J.~G.~Lu$^{1,50}$, X.~L.~Lu$^{1}$, Y.~Lu$^{1}$, Y.~P.~Lu$^{1,50}$, C.~L.~Luo$^{34}$, M.~X.~Luo$^{72}$, T.~Luo$^{9,g}$, X.~L.~Luo$^{1,50}$, X.~R.~Lyu$^{55}$, F.~C.~Ma$^{33}$, H.~L.~Ma$^{1}$, L.~L.~Ma$^{42}$, M.~M.~Ma$^{1,55}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,55}$, R.~T.~Ma$^{55}$, X.~X.~Ma$^{1,55}$, X.~Y.~Ma$^{1,50}$, Y.~Ma$^{39,h}$, F.~E.~Maas$^{14}$, M.~Maggiora$^{67A,67C}$, S.~Maldaner$^{4}$, S.~Malde$^{62}$, Q.~A.~Malik$^{66}$, A.~Mangoni$^{23B}$, Y.~J.~Mao$^{39,h}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{67A,67C}$, Z.~X.~Meng$^{58}$, J.~G.~Messchendorp$^{56,d}$, G.~Mezzadri$^{24A}$, T.~J.~Min$^{35}$, R.~E.~Mitchell$^{22}$, X.~H.~Mo$^{1,50,55}$, N.~Yu.~Muchnoi$^{10,b}$, H.~Muramatsu$^{60}$, S.~Nakhoul$^{11,e}$, Y.~Nefedov$^{29}$, F.~Nerling$^{11,e}$, I.~B.~Nikolaev$^{10,b}$, Z.~Ning$^{1,50}$, S.~Nisar$^{8,m}$, S.~L.~Olsen$^{55}$, Q.~Ouyang$^{1,50,55}$, S.~Pacetti$^{23B,23C}$, X.~Pan$^{9,g}$, Y.~Pan$^{59}$, A.~Pathak$^{1}$, A.~~Pathak$^{27}$, P.~Patteri$^{23A}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{64,50}$, K.~Peters$^{11,e}$, J.~Pettersson$^{68}$, J.~L.~Ping$^{34}$, R.~G.~Ping$^{1,55}$, S.~Plura$^{28}$, S.~Pogodin$^{29}$, R.~Poling$^{60}$, V.~Prasad$^{64,50}$, H.~Qi$^{64,50}$, H.~R.~Qi$^{53}$, M.~Qi$^{35}$, T.~Y.~Qi$^{9,g}$, S.~Qian$^{1,50}$, W.~B.~Qian$^{55}$, Z.~Qian$^{51}$, C.~F.~Qiao$^{55}$, J.~J.~Qin$^{65}$, L.~Q.~Qin$^{12}$, X.~P.~Qin$^{9,g}$, X.~S.~Qin$^{42}$, Z.~H.~Qin$^{1,50}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{36}$, K.~H.~Rashid$^{66}$, K.~Ravindran$^{21}$, C.~F.~Redmer$^{28}$, A.~Rivetti$^{67C}$, V.~Rodin$^{56}$, M.~Rolo$^{67C}$, G.~Rong$^{1,55}$, Ch.~Rosner$^{14}$, M.~Rump$^{61}$, H.~S.~Sang$^{64}$, A.~Sarantsev$^{29,c}$, Y.~Schelhaas$^{28}$, C.~Schnier$^{4}$, K.~Schoenning$^{68}$, M.~Scodeggio$^{24A,24B}$, W.~Shan$^{19}$, X.~Y.~Shan$^{64,50}$, J.~F.~Shangguan$^{47}$, M.~Shao$^{64,50}$, C.~P.~Shen$^{9,g}$, H.~F.~Shen$^{1,55}$, X.~Y.~Shen$^{1,55}$, H.~C.~Shi$^{64,50}$, R.~S.~Shi$^{1,55}$, X.~Shi$^{1,50}$, X.~D~Shi$^{64,50}$, J.~J.~Song$^{15}$, W.~M.~Song$^{27,1}$, Y.~X.~Song$^{39,h}$, S.~Sosio$^{67A,67C}$, S.~Spataro$^{67A,67C}$, F.~Stieler$^{28}$, K.~X.~Su$^{69}$, P.~P.~Su$^{47}$, G.~X.~Sun$^{1}$, H.~K.~Sun$^{1}$, J.~F.~Sun$^{15}$, L.~Sun$^{69}$, S.~S.~Sun$^{1,55}$, T.~Sun$^{1,55}$, W.~Y.~Sun$^{27}$, X~Sun$^{20,i}$, Y.~J.~Sun$^{64,50}$, Y.~Z.~Sun$^{1}$, Z.~T.~Sun$^{42}$, Y.~H.~Tan$^{69}$, Y.~X.~Tan$^{64,50}$, C.~J.~Tang$^{46}$, G.~Y.~Tang$^{1}$, J.~Tang$^{51}$, J.~X.~Teng$^{64,50}$, V.~Thoren$^{68}$, W.~H.~Tian$^{44}$, Y.~T.~Tian$^{25}$, I.~Uman$^{54B}$, B.~Wang$^{1}$, C.~W.~Wang$^{35}$, D.~Y.~Wang$^{39,h}$, H.~J.~Wang$^{31,k,l}$, H.~P.~Wang$^{1,55}$, K.~Wang$^{1,50}$, L.~L.~Wang$^{1}$, M.~Wang$^{42}$, M.~Z.~Wang$^{39,h}$, Meng~Wang$^{1,55}$, S.~Wang$^{9,g}$, W.~Wang$^{51}$, W.~H.~Wang$^{69}$, W.~P.~Wang$^{64,50}$, X.~Wang$^{39,h}$, X.~F.~Wang$^{31,k,l}$, X.~L.~Wang$^{9,g}$, Y.~D.~Wang$^{38}$, Y.~F.~Wang$^{1,50,55}$, Y.~Q.~Wang$^{1}$, Y.~Y.~Wang$^{31,k,l}$, Ying~Wang$^{51}$, Z.~Wang$^{1,50}$, Z.~Y.~Wang$^{1}$, Ziyi~Wang$^{55}$, Zongyuan~Wang$^{1,55}$, D.~H.~Wei$^{12}$, F.~Weidner$^{61}$, S.~P.~Wen$^{1}$, D.~J.~White$^{59}$, U.~Wiedner$^{4}$, G.~Wilkinson$^{62}$, M.~Wolke$^{68}$, L.~Wollenberg$^{4}$, J.~F.~Wu$^{1,55}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,55}$, X.~Wu$^{9,g}$, X.~H.~Wu$^{27}$, Z.~Wu$^{1,50}$, L.~Xia$^{64,50}$, T.~Xiang$^{39,h}$, H.~Xiao$^{9,g}$, S.~Y.~Xiao$^{1}$, Z.~J.~Xiao$^{34}$, X.~H.~Xie$^{39,h}$, Y.~G.~Xie$^{1,50}$, Y.~H.~Xie$^{6}$, T.~Y.~Xing$^{1,55}$, C.~J.~Xu$^{51}$, G.~F.~Xu$^{1}$, Q.~J.~Xu$^{13}$, S.~Y.~Xu$^{63}$, W.~Xu$^{1,55}$, X.~P.~Xu$^{47}$, Y.~C.~Xu$^{55}$, F.~Yan$^{9,g}$, L.~Yan$^{9,g}$, W.~B.~Yan$^{64,50}$, W.~C.~Yan$^{73}$, H.~J.~Yang$^{43,f}$, H.~X.~Yang$^{1}$, L.~Yang$^{44}$, S.~L.~Yang$^{55}$, Yifan~Yang$^{1,55}$, Zhi~Yang$^{25}$, M.~Ye$^{1,50}$, M.~H.~Ye$^{7}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{51}$, B.~X.~Yu$^{1,50,55}$, C.~X.~Yu$^{36}$, G.~Yu$^{1,55}$, J.~S.~Yu$^{20,i}$, T.~Yu$^{65}$, C.~Z.~Yuan$^{1,55}$, L.~Yuan$^{2}$, X.~Q.~Yuan$^{1}$, Y.~Yuan$^{1}$, Z.~Y.~Yuan$^{51}$, C.~X.~Yue$^{32}$, A.~A.~Zafar$^{66}$, X.~Zeng~Zeng$^{6}$, Y.~Zeng$^{20,i}$, A.~Q.~Zhang$^{1}$, B.~X.~Zhang$^{1}$, G.~Y.~Zhang$^{15}$, H.~Zhang$^{64}$, H.~H.~Zhang$^{27}$, H.~H.~Zhang$^{51}$, H.~Y.~Zhang$^{1,50}$, J.~L.~Zhang$^{70}$, J.~Q.~Zhang$^{34}$, J.~W.~Zhang$^{1,50,55}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,55}$, Jianyu~Zhang$^{1,55}$, Jiawei~Zhang$^{1,55}$, L.~M.~Zhang$^{53}$, L.~Q.~Zhang$^{51}$, Lei~Zhang$^{35}$, S.~F.~Zhang$^{35}$, Shulei~Zhang$^{20,i}$, X.~D.~Zhang$^{38}$, X.~Y.~Zhang$^{42}$, Y.~Zhang$^{62}$, Y. ~T.~Zhang$^{73}$, Y.~H.~Zhang$^{1,50}$, Yan~Zhang$^{64,50}$, Yao~Zhang$^{1}$, Z.~Y.~Zhang$^{69}$, G.~Zhao$^{1}$, J.~Zhao$^{32}$, J.~Y.~Zhao$^{1,55}$, J.~Z.~Zhao$^{1,50}$, Lei~Zhao$^{64,50}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{36}$, Q.~Zhao$^{1}$, S.~J.~Zhao$^{73}$, Y.~B.~Zhao$^{1,50}$, Y.~X.~Zhao$^{25}$, Z.~G.~Zhao$^{64,50}$, A.~Zhemchugov$^{29,a}$, B.~Zheng$^{65}$, J.~P.~Zheng$^{1,50}$, Y.~H.~Zheng$^{55}$, B.~Zhong$^{34}$, C.~Zhong$^{65}$, L.~P.~Zhou$^{1,55}$, Q.~Zhou$^{1,55}$, X.~Zhou$^{69}$, X.~K.~Zhou$^{55}$, X.~R.~Zhou$^{64,50}$, X.~Y.~Zhou$^{32}$, A.~N.~Zhu$^{1,55}$, J.~Zhu$^{36}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,50,55}$, S.~H.~Zhu$^{63}$, T.~J.~Zhu$^{70}$, W.~J.~Zhu$^{36}$, W.~J.~Zhu$^{9,g}$, Y.~C.~Zhu$^{64,50}$, Z.~A.~Zhu$^{1,55}$, B.~S.~Zou$^{1}$, J.~H.~Zou$^{1}$\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
$^{4}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{8}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{9}$ Fudan University, Shanghai 200443, People's Republic of China\\
$^{10}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{11}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{12}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{13}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{14}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{15}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{16}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{17}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{18}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{19}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{20}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{21}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{22}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{23}$ INFN Laboratori Nazionali di Frascati , (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{24}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{25}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{26}$ Institute of Physics and Technology, Peace Ave. 54B, Ulaanbaatar 13330, Mongolia\\
$^{27}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{28}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{29}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{30}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{31}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{32}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{33}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{34}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{35}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{36}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{37}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{38}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{39}$ Peking University, Beijing 100871, People's Republic of China\\
$^{40}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{41}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{42}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{43}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{44}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{45}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{46}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{47}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{48}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{49}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{50}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{51}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{52}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{53}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{54}$ Turkish Accelerator Center Particle Factory Group, (A)Istinye University, 34010, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, Mersin 10, Turkey\\
$^{55}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{56}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{57}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{58}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{59}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{60}$ University of Minnesota, Minneapolis, Minnesota 55455, USA\\
$^{61}$ University of Muenster, Wilhelm-Klemm-Str. 9, 48149 Muenster, Germany\\
$^{62}$ University of Oxford, Keble Rd, Oxford, UK OX13RH\\
$^{63}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{64}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{65}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{66}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{67}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{68}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{69}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{70}$ Xinyang Normal University, Xinyang 464000, People's Republic of China\\
$^{71}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{72}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{73}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{b}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{c}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{d}$ Currently at Istanbul Arel University, 34295 Istanbul, Turkey\\
$^{e}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{f}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{g}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{h}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{i}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{j}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{k}$ Also at Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{l}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{m}$ Also at the Department of Mathematical Sciences, IBA, Karachi , Pakistan\\
}\vspace{0.4cm}}


